Efficient Interaction-Based Offline Runtime Verification of Distributed Systems with Lifeline Removal

Runtime Verification (RV) refers to a family of techniques in which system executions are observed and confronted to formal specifications, with the aim of identifying faults. In Offline RV, observation is done in a first step and verification in a second, on a static artifact collected during observation. In this paper, we define an approach to offline RV of Distributed Systems (DS) against interactions. Interactions are formal models describing communications within a DS. DS are composed of subsystems deployed on different machines and interacting via message passing. Therefore, observing executions of a DS entails logging a collection of local execution traces, one for each subsystem, that we call a multi-trace. A major challenge in analyzing multi-traces is that there are no practical means to synchronize the ends of observations of all local traces. We address this via an operation, called lifeline removal, which we apply on-the-fly on the specification during verification once a local trace has been entirely analyzed. This operation removes from the interaction the specification of actions occurring on the subsystem that is no-longer observed. This may allow further execution of the specification via removing deadlocks due to the partial orders of actions. We prove the correctness of the resulting RV algorithm and introduce two optimization techniques which we also prove correct. We implement a Partial Order Reduction (POR) technique via the selection of a one-unambiguous action (as a unique first step to a linearization) which existence is determined via another use of the lifeline removal operator. Additionally, Local Analyses (LOC) i.e., the verification of local traces, can be leveraged during the global multi-trace analysis to prove failure more quickly. Experiments illustrate the application of our RV approach and the benefits of our optimizations.

==> appendices/A2_3.tex <==

\subsection{Collision and Pruning}

The execution relation $\rightarrow$ relies on the definition of two other inductive predicates: collision and pruning.
The collision predicate $\collidesLf$ is such that $i \collidesLf l$ signifies that all traces of $i$ have at least an action occurring on the lifeline $l$. 

\begin{definition}[Collision]\label{def:collision}
The predicate $\collidesLf \subset \mathbb{I}(L) \times L$ is such that for $i_1$ and $i_2$ in $\mathbb{I}(L)$, $l\in L$, $a \in \mathbb{A}(L)$ and $f \in \{strict,seq,par\}$ we have:

{
\centering
%
\begin{minipage}{2cm}
\begin{prooftree}
\AxiomC{$\theta(a) = l$}
\UnaryInfC{$a \collidesLf l$}
\end{prooftree}
\end{minipage}
%
\vspace*{.1cm}
\begin{minipage}{3.5cm}
\begin{prooftree}
\AxiomC{$i_1 \collidesLf l$}
\AxiomC{$i_2 \collidesLf l$}
\BinaryInfC{$alt(i_1,i_2) \collidesLf l$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{2.75cm}
\begin{prooftree}
\AxiomC{$i_1 \collidesLf l$}
\UnaryInfC{$f(i_1,i_2) \collidesLf l$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{2.75cm}
\begin{prooftree}
\AxiomC{$i_2 \collidesLf l$}
\UnaryInfC{$f(i_1,i_2) \collidesLf l$}
\end{prooftree}
\end{minipage}
%
}
\end{definition}





\begin{property}
\label{prop:collision_and_lifeline_removal_2}
For all $l \in L \setminus H$ and for all $i \in \mathbb{I}(L)$ we have:
$(i \collidesLf l) \Rightarrow (i_h \collidesLf l)$
%$(i_h \collidesLf l) \Rightarrow (i \collidesLf l)$
\end{property}

\begin{proof}
%try
Let us prove $\varphi$ : $(i \collidesLf l) \Rightarrow (i_h \collidesLf l)$ by induction.

%$l \in L \setminus H$
Let us reason on the form of $i$:
\begin{itemize}

\item If $i = \varnothing$ then $i_h = \varnothing$ the premise of $\varphi$ does not hold, therefore $\varphi$ holds.

\item If $i =  a \in \mathbb{A}(L)$  and $(i \collidesLf l)$, then $\theta(a) = l$ . Since $l \not\in H$, then $i_h = i$, and therefore $(i_h \collidesLf l)$. Thus $\varphi$ holds.

\end{itemize}

The remaining of the proof consists of trivial induction steps where for each term of the form $f(i_1,i_2)$, the induction hypotheses, being either
$(t_1 \collidesLf l) \Rightarrow ({t_1}_h \collidesLf l)$, or $(t_2 \collidesLf l) \Rightarrow ({t_2}_h \collidesLf l)$, or the conjunction of both depending on the form of $f$, trivially imply that $\varphi$ holds.   


%By induction of the term structure of $i$.
%If $i = \varnothing$ then $i_h = \varnothing$ %the premise does not hold.
%If $i = a \in \mathbb{A}(L)$ then:
%\begin{itemize}
%    \item if $\theta(a) \in H$, we have $i_h = \varnothing$ and the premise does not hold
%    \item otherwise, we have $i_h = i$ and %the conclusion trivially holds
%\end{itemize}

%Given $i_1$ and $i_2$ two interactions, if $i=f(i_1,i_2)$ with $f \in \{strict,seq,par\}$ a scheduling operator then $i_h = f(i_{1h},i_{2h})$ and $i_h \collidesLf l$ iff either (or both of) $i_{1h} \collidesLf l$ or $i_{2h} \collidesLf l$. Let us suppose the former, all other things being equivalent.
%By induction, the fact that $i_{1h} \collidesLf l$ implies that $i_1 \collidesLf l$ and therefore that $i \collidesLf l$.
%For $i=alt(i_1,i_2)$, we reason similarly (except that it is a logic AND instead of OR).
%If $i = loop_k(i_1)$, with $k \in \{S,W,P\}$, we have $i_h = loop_k(i_{1h})$ and the premise does not hold.
\end{proof}



Pruning $i \isPruneOf{l} i'$ is defined so that $i'$ characterizes the maximum subset of accepted traces by $i$ that contains no trace with actions on $l$.

\begin{definition}[Pruning]\label{def:pruning_relation}
The pruning relation $\isPruneBase \; \subset \mathbb{I}(L) \times L \times \mathbb{I}(L)$ is s.t. for any $l \in L$, any $f \in \{strict,seq,par\}$ and any $k \in \{S,W,P\}$:

{
\centering
\begin{minipage}{2.5cm}
\begin{prooftree}
\AxiomC{\vphantom{$\isPruneOf{l}$}}
\UnaryInfC{$\varnothing \isPruneOf{l} \varnothing$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{2.5cm}
\begin{prooftree}
\AxiomC{\vphantom{$\theta(a) \neq l$} \vphantom{$\isPruneOf{l}$}}
\RightLabel{$\theta(a) \neq l$}
\UnaryInfC{$a \isPruneOf{l} a$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{4cm}
\begin{prooftree}
\AxiomC{$i_1 \isPruneOf{l} i_1'$}
\AxiomC{$i_2 \isPruneOf{l} i_2'$}
\BinaryInfC{$f(i_1,i_2) \isPruneOf{l} f(i_1',i_2')$}
\end{prooftree}
\end{minipage}

\vspace*{.1cm}

\begin{minipage}{3.85cm}
\begin{prooftree}
\AxiomC{$i_1 \isPruneOf{l} i_1'$}
\AxiomC{$i_2 \isPruneOf{l} i_2'$}
\BinaryInfC{$alt(i_1,i_2) \isPruneOf{l} alt(i_1',i_2')$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{3.85cm}
\begin{prooftree}
\AxiomC{$i_1 \isPruneOf{l} i_1'$}
\RightLabel{$i_2 \collidesLf l$}
\UnaryInfC{$alt(i_1,i_2) \isPruneOf{l} i_1'$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{3.85cm}
\begin{prooftree}
\AxiomC{$i_2 \isPruneOf{l} i_2'$}
\RightLabel{$i_1 \collidesLf l$}
\UnaryInfC{$alt(i_1,i_2) \isPruneOf{l} i_2'$}
\end{prooftree}
\end{minipage}

\vspace*{.1cm}

\begin{minipage}{5cm}
\begin{prooftree}
\AxiomC{$i_1 \isPruneOf{l} i_1'$}
\UnaryInfC{$loop_k(i_1) \isPruneOf{l} loop_k(i_1')$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{5cm}
\begin{prooftree}
\AxiomC{$\phantom{\isPruneOf{l}}$}
\RightLabel{$i_1 \collidesLf l$}
\UnaryInfC{$loop_k(i_1) \isPruneOf{l} \varnothing$}
\end{prooftree}
\end{minipage}
\\
}
\end{definition}




\begin{property}
\label{prop:pruning_and_lifeline_removal}
Let $l \not\in H$.
$i \isPruneOf{l}  i' \Rightarrow i_h \isPruneOf{l}  i'_h$. 
\end{property}

\begin{proof}

Let us prove $\varphi$ : $i \isPruneOf{l}  i' \Rightarrow i_h \isPruneOf{l}  i'_h$ by induction.

Let us reason on the form of $i$:
\begin{itemize}

\item 
If $i = \varnothing$ then $i'=\varnothing$, $i_h=\varnothing$ and  
$i_h \isPruneOf{l} \varnothing$, that is $i_h \isPruneOf{l} i'_h$, therefore $\varphi$ holds.

\item If $i =  a \in \mathbb{A}(L)$ then $i \isPruneOf{l}  i'$ implies $\theta(a) \neq l$ and $i'=a$. If $\theta(a)\in H$ then $i_h=\varnothing$ 
and $i_h \isPruneOf{l} \varnothing$, that is $i_h \isPruneOf{l} i'_h$, therefore $\varphi$ holds. If $\theta(a)\notin H$ then $i_h=a$
and $i_h \isPruneOf{l} a$, that is $i_h \isPruneOf{l} i'_h$, therefore $\varphi$ holds.

\end{itemize}

The remaining of the proof is conducted by induction on $i$, using the rules of Def.\ref{def:pruning_relation} that relate to the root operator of $i$, and supposing that $\varphi$ holds for the sub-terms of $i$. For each rule, the conclusion that $\varphi$ holds comes immediately (using Prop.\ref{prop:collision_and_lifeline_removal_2} in the case of $alt$ and $loop_k$).



\end{proof}









==> appendices/A2_4.tex <==

\subsection{Execution}





The execution relation (Def.\ref{def:execution_relation} below) relates a term $i$ with a follow-up term $i'$ that results from executing an action $a$ at a specific position $p$ in $i$. 

\begin{definition}
\label{def:execution_relation}
Given $i_1$, $i_2$, $i_1'$ and $i_2'$ interactions in $\mathbb{I}(L)$, $a$ an action in $\mathbb{A}(L)$ and $p$ a position in $\{1,2\}^*$, the execution relation $\rightarrow \subset \mathbb{I}(L) \times \{1,2\}^* \times \mathbb{A}(L)  \times \mathbb{I}(L)$ is s.t.:

{
\centering
%act
\begin{minipage}{3cm}
\begin{prooftree}
\AxiomC{\phantom{$\xrightarrow{a@p}$}}
\UnaryInfC{$a \xrightarrow{a@\varepsilon} \varnothing$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{3.5cm}
\begin{prooftree}
\AxiomC{$i_1 \xrightarrow{a@p} i'_1$}
\UnaryInfC{$alt(i_1,i_2) \xrightarrow{a@1p} i'_1$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{3.5cm}
\begin{prooftree}
\AxiomC{$i_2 \xrightarrow{a@p} i'_2$}
\UnaryInfC{$alt(i_1,i_2) \xrightarrow{a@2p} i'_2$}
\end{prooftree}
\end{minipage}

\vspace{0.1cm}

% par
\begin{minipage}{5.5cm}
\begin{prooftree}
\AxiomC{$i_1 \xrightarrow{a@p} i'_1$}
\UnaryInfC{$par(i_1,i_2) \xrightarrow{a@1p} par(i'_1,i_2)$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{5.5cm}
\begin{prooftree}
\AxiomC{$i_2 \xrightarrow{a@p} i'_2$}
\UnaryInfC{$par(i_1,i_2) \xrightarrow{a@2p} par(i_1,i'_2)$}
\end{prooftree}
\end{minipage}

\vspace{0.1cm}

% strict  
\begin{minipage}{5.5cm}
\begin{prooftree}
\AxiomC{$i_1 \xrightarrow{a@p} i'_1$}
\UnaryInfC{$strict(i_1,i_2) \xrightarrow{a@1p} strict(i'_1,i_2)$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{5.5cm}
\begin{prooftree}
\AxiomC{$i_2 \xrightarrow{a@p} i'_2$}
\RightLabel{$i_1 \downarrow$}
\UnaryInfC{$strict(i_1,i_2) \xrightarrow{a@2p} i'_2$}
\end{prooftree}
\end{minipage}

\vspace{0.1cm}

% seq  
\begin{minipage}{5.5cm}
\begin{prooftree}
\AxiomC{$i_1 \xrightarrow{a@p} i'_1$}
\UnaryInfC{$seq(i_1,i_2) \xrightarrow{a@1p} seq(i'_1,i_2)$}
\end{prooftree}
\end{minipage}
%
\begin{minipage}{5.5cm}
\begin{prooftree}
\AxiomC{$i_1 \isPruneOf{\theta(a)} i_1'$}
\AxiomC{$i_2 \xrightarrow{a@p} i_2'$}
\BinaryInfC{$seq(i_1,i_2) \xrightarrow{a@2p} seq(i_1',i_2')$}
\end{prooftree}
\end{minipage}

\vspace{0.1cm}

\begin{minipage}{8cm}
\begin{prooftree}
\AxiomC{$i_1 \xrightarrow{a@p} i_1'$}
\UnaryInfC{$loop_S(i_1) \xrightarrow{a@1p} strict(i_1',loop_S(i_1))$}
\end{prooftree}
\end{minipage}
 
\vspace{0.1cm}
 
\begin{minipage}{8cm}
\begin{prooftree}
\AxiomC{$i_1 \xrightarrow{a@p} i_1'$}
\AxiomC{$loop_W(i_1) \isPruneOf{\theta(a)} i'$}
\BinaryInfC{$loop_W(i_1) \xrightarrow{a@1p} seq(i',seq(i_1',loop_W(i_1)))$}
\end{prooftree}
\end{minipage}

\vspace{0.1cm}

\begin{minipage}{8cm}
\begin{prooftree}
\AxiomC{$i_1 \xrightarrow{a@p} i_1'$}
\UnaryInfC{$loop_P(i_1) \xrightarrow{a@1p} par(i_1',loop_P(i_1))$}
\end{prooftree}
\end{minipage}\\
}

\end{definition}


We prove below Prop.\ref{prop:execution_and_lifeline_removal} from Sec.\ref{sec:semantics} which relates the execution relation to the lifeline removal operator.


\begin{property*}[Prop.\ref{prop:execution_and_lifeline_removal}, Sec.\ref{sec:semantics}]
For any $L \subset \mathcal{L}$, any interaction $i \in \mathbb{I}(L)$, any set of lifelines $\emptyset \subsetneq H \subsetneq L$, any action $a \in \mathbb{A}(L)$ s.t.~$\theta(a) \not\in H$ and any position $p \in pos(i)$:
\[
(\exists~i' \in \mathbb{I}(L),~i \xrightarrow{a@p} i') ~\Rightarrow~ (i_h \xrightarrow{a@p} i'_h)
\]
\end{property*}




\begin{proof}




Let us prove $\varphi$ : 

\[
(\exists~i' \in \mathbb{I}(L),~i \xrightarrow{a@p} i') ~\Rightarrow~ (i_h \xrightarrow{a@p} i'_h)
\] 
 
 by induction.

%$l \in L \setminus H$
Let us reason on the form of $i$:
\begin{itemize}

\item 
If $i = \varnothing$ then the premise of $\varphi$ dos not hold. Therefore $\varphi$ holds.

\item If $i =  a \in \mathbb{A}(L)$ then 
$p=\varepsilon$ and $i'=\varnothing$. Then, because $\theta(a) \not\in H$, we have $i_h = a$ and $i'_h = \varnothing$ which satisfies $i_h \xrightarrow{a@\varepsilon} i'_h$. Therefore $\varphi$ holds. 

\end{itemize}

The remaining of the proof is conducted by induction on the form of $i$, using the rules of Def.\ref{def:execution_relation} that relate to the root operator of $i$, and supposing that $\varphi$ holds for the sub-terms of $i$, as defined in the corresponding rule. For each rule, the conclusion that $\varphi$ holds comes immediately (using  Prop.\ref{prop:termination_and_lifeline_removal}  (resp. Prop.\ref{prop:pruning_and_lifeline_removal}) in the case of $strict$ (resp. $seq$)  when executing an action in the right sub-term).









\iffalse

Let us suppose $i \xrightarrow{a@p} i'$ and reason by induction on the term structure of $i$.
We cannot have $i = \varnothing$ as the premise would not hold.
If $i \in \mathbb{A}(L)$ then $a = i$, $p = \varepsilon$ and $i' = \varnothing$. Then, because $\theta(a) \not\in H$, we have $i_h = a$ and $i'_h = \varnothing$ which satisfies $i_h \xrightarrow{a@\varepsilon} i'_h$.

Given $i_1$ and $i_2$ two interactions, if $i = f(i_1,i_2)$ with $f \in \{strict,seq,par,alt\}$ any binary operator, the fact that $i \xrightarrow{a@p}$ implies that $p$ is
\begin{itemize}
    \item either of the form $1.p_1$ and we have a $i_1'$ s.t., $i_1 \xrightarrow{a@p_1} i_1'$, and then, by induction, we have $i_{1h} \xrightarrow{a@p_1} i'_{1h}$
    \item or of the form $2.p_2$ and we have a $i_2'$ s.t., $i_2 \xrightarrow{a@p_2} i_2'$, and then, by induction, we have $i_{2h} \xrightarrow{a@p_2} i'_{2h}$
\end{itemize}

 Then:
\begin{itemize}
    \item if $i = alt(i_1,i_2)$, supposing the action is on the side of $i_1$ (the other case being symmetric), we have $i \xrightarrow{a@1.p_1} i_1'$. Then, because by induction we have $i_{1h} \xrightarrow{a@p_1} i'_{1h}$, by Def.\ref{def:execution_relation}, this implies $alt(i_{1h},i_{2h}) \xrightarrow{a@1.p_1} i'_{1h}$ and thus $i_h \xrightarrow{a@p} i'_h$
    \item if $i = strict(i_1,i_2)$:
    \begin{itemize}
        \item if the action comes from $i_1$ then we have $i \xrightarrow{a@1.p_1} strict(i_1',i_2)$ and via induction and Def.\ref{def:execution_relation}, $strict(i_{1h},i_{2h}) \xrightarrow{a@1.p_1} strict(i'_{1h},i_{2h})$ hence, via Def.\ref{def:lifeline_removal_operator_on_interactions} the property holds
        \item if the action comes from $i_2$ then we have $i \xrightarrow{a@2.p_2} i'_2$ and $i_1 \downarrow$. As per Prop.\ref{prop:termination_and_lifeline_removal}, we also have $i_{1h} \downarrow$. Hence, via induction and Def.\ref{def:execution_relation}, $strict(i_{1h},i_{2h}) \xrightarrow{a@2.p_2} i'_{2h}$ hence, via Def.\ref{def:lifeline_removal_operator_on_interactions} the property holds
    \end{itemize}
    \item if $i = par(i_1,i_2)$ we reason as in the first case of $strict$
    \item if $i = seq(i_1,i_2)$, let us consider the case where the action comes from $i_2$ (the other being similar to the first case of $strict$). Then we must have $i_1 \isPruneOf{\theta(a)} i_1'$ and $i_2 \xrightarrow{a@p_2} i_2'$.
    Via Prop.\ref{prop:pruning_and_lifeline_removal}, and given $\theta(a) \not\in H$, the former implies $i_{1h} \isPruneOf{\theta(a)} i'_{1h}$, and, via induction, the latter implies $i_{2h} \xrightarrow{a@p_2} i'_{2h}$. Hence, as per Def.\ref{def:execution_relation}, we have $seq(i_{1h},i_{2h}) \xrightarrow{a@2.p_2} seq(i'_{1h},i'_{2h})$ and thus, via Def.\ref{def:lifeline_removal_operator_on_interactions} the property holds.
\end{itemize}

In the case of loops, for a derivation $loop_k(i_1) \xrightarrow{a@p} x$ to exist (given $k \in \{S,W,P\}$), we must have $p$ of the form $1.p_1$ and there must exist a $i'_1$ s.t.~$i_1 \xrightarrow{a@p_1} i_1'$, which, by induction, implies $i_{1h} \xrightarrow{a@p_1} i'_{1h}$.
Then:
\begin{itemize}
    \item in the case $(k,f) \in \{(S,strict),(P,par)\}$, we have $i = loop_k(i_1) \xrightarrow{a@1.p_1} f(i_1',i)$. Because by induction we have $i_{1h} \xrightarrow{a@p_1} i'_{1h}$, we also have $loop_k(i_{1h}) \xrightarrow{a@1.p_1} f(i'_{1h},loop_k(i_{1h}))$ and because by Def.\ref{def:lifeline_removal_operator_on_interactions} we have $i_h = loop_k(i_{1h})$, the property holds.
    \item in the case $i = loop_W(i_1)$, there exists a $i'$ s.t.~$i \isPruneOf{\theta(a)} i'$ and we have $i \xrightarrow{a@1.p_1} seq(i',seq(i_1',i))$. Via Prop.\ref{prop:pruning_and_lifeline_removal}, and because $\theta(a) \not\in H$, we have $i_h \isPruneOf{\theta(a)} i'_h$. Hence, because $i_h = loop_W(i_{1h})$ (Def.\ref{def:lifeline_removal_operator_on_interactions}) and because by induction we have $i_{1h} \xrightarrow{a@p_1} i'_{1h}$, we also (Def.\ref{def:execution_relation}) have $loop_W(i_{1h}) \xrightarrow{a@1.p_1} seq(i'_h,seq(i'_{1h},i_h))$. Thus the property holds.
\end{itemize}
\fi


\end{proof}




==> figures/subfig/tikz_l1.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {$\hlf{l_p}$};
    \node[below=.1cm of lab] (img) {\includegraphics[height=1.4cm]{images/icons/icon_device.png}};
\end{tikzpicture}

==> figures/subfig/tikz_l2.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {$\hlf{l_b}$};
    \node[below=.1cm of lab] (img) {\includegraphics[width=1.6cm]{images/icons/icon_server.png}};
\end{tikzpicture}

==> figures/subfig/tikz_l3.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {$\hlf{l_s}$};
    \node[below=.1cm of lab] (img) {\includegraphics[height=1.3cm]{images/icons/icon_smartphone.png}};
\end{tikzpicture}

==> figures/subfig/tikz_pub_bro_sub.tex <==
\begin{tikzpicture}
\tikzstyle{subsys}=[draw,hibou_col_lf,rectangle,line width=2pt,minimum height=2cm,minimum width=2cm,inner sep=0,outer sep=0]
%
\node[subsys] (A) at (-1.5,0) {
    \input{figures/subfig/tikz_l1}
};
%
\node[subsys] (B) at (1.5,1.5) {
    \input{figures/subfig/tikz_l2}
};
%
\node[subsys] (C) at (1.25,-1) {
    \input{figures/subfig/tikz_l3}
};
%
\draw[<->,line width=2.5pt,hibou_col_ms] (A) -- (B);
\draw[<->,line width=2.5pt,hibou_col_ms] (A) -- (C);
\draw[<->,line width=2.5pt,hibou_col_ms] (C) -- (B);
\end{tikzpicture}

==> figures/subfig/tikz_reord.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {\small\texttt{reordering}};
    \node[below=.1cm of lab] (img) {\includegraphics[height=1.3cm]{images/icons/icon_ordering.png}};
\end{tikzpicture}

==> images/locana_basic_fail/locana_l1.tex <==
\begin{tikzpicture}
\node[draw,black] (s1_l1_0) {
    \begin{tikzpicture}
    \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/projl1_1.png}};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_1}\} \leftarrow \hlf{l_1}!\hms{m_1}.\hlf{l_1}!\hms{m_2}.\hlf{l_1}!\hms{m_3}$
    };
    \end{tikzpicture}
    };
%
\node[draw,black, right=.75cm of s1_l1_0] (s1_l1_1) {
    \begin{tikzpicture}
    \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/projl1_2.png}};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_1}\} \leftarrow \hlf{l_1}!\hms{m_2}.\hlf{l_1}!\hms{m_3}$
    };
    \end{tikzpicture}
};
\draw[->,black] (s1_l1_0) -- node[midway,fill=white,draw=black,rotate=90] {\footnotesize$\hlf{l_1}!\hms{m_1}$} (s1_l1_1);
%
\node[draw,black, right=.75cm of s1_l1_1] (s1_l1_2) {
    \begin{tikzpicture}
    \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/projl1_3.png}};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_1}\} \leftarrow \hlf{l_1}!\hms{m_3}$
    };
    \end{tikzpicture}
};
\draw[->,black] (s1_l1_1) -- node[midway,fill=white,draw=black,rotate=90] {\footnotesize$\hlf{l_1}!\hms{m_2}$} (s1_l1_2);
%
\node[draw,black, right=.75cm of s1_l1_2] (s1_l1_3) {
    \begin{tikzpicture}
    \node (int) {$\varnothing$};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_1}\} \leftarrow \varepsilon$
    };
    \end{tikzpicture}
};
\draw[->,black] (s1_l1_2) -- node[midway,fill=white,draw=black,rotate=90] {\footnotesize$\hlf{l_1}!\hms{m_3}$} (s1_l1_3);
%
\node[draw,black, below=.25cm of s1_l1_3,chamfered rectangle,fill=blue,minimum width=1.5cm,minimum height=.5cm] (v) {\textcolor{white}{\textbf{Ok}}};
\draw[->,blue] (s1_l1_3) -- (v);
\end{tikzpicture}

==> images/locana_basic_fail/locana_l2.tex <==
\begin{tikzpicture}
    \node[draw,black] (s1_l2_0) {
        \begin{tikzpicture}
        \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/isd4.png}};
        \node[right=-.25cm of int,align=left] (mu) {
        $\{\hlf{l_2}\} \leftarrow \hlf{l_2}!\hms{m_3}$
        };
        \end{tikzpicture}
    };
    \node[draw,black, right=.75cm of s1_l2_0,chamfered rectangle,fill=red,minimum width=1.5cm,minimum height=.5cm] (v_1_l2) {\textcolor{white}{\textbf{Nok}}};
    \draw[->,red] (s1_l2_0) -- (v_1_l2);
\end{tikzpicture}

==> images/locana_basic_fail/noloc.tex <==
\begin{tikzpicture}
\node[draw] (s0) {
    \begin{tikzpicture}
    \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/isd1.png}};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_1}\} \leftarrow \hlf{l_1}!\hms{m_1}.\hlf{l_1}!\hms{m_2}.\hlf{l_1}!\hms{m_3}$\\
    $\{\hlf{l_2}\} \leftarrow \hlf{l_2}!\hms{m_3}$
    };
    \end{tikzpicture}
    };
%
\node[draw, right=.75cm of s0] (s1) {
    \begin{tikzpicture}
    \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/isd2.png}};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_1}\} \leftarrow \hlf{l_1}!\hms{m_2}.\hlf{l_1}!\hms{m_3}$\\
    $\{\hlf{l_2}\} \leftarrow \hlf{l_2}!\hms{m_3}$
    };
    \end{tikzpicture}
};
\draw[->] (s0) -- node[midway,fill=white,draw,rotate=90] {\footnotesize$\hlf{l_1}!\hms{m_1}$} (s1);
%
\node[draw, below=.75cm of s1.south east,anchor=north east] (s2) {
    \begin{tikzpicture}
    \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/isd3.png}};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_1}\} \leftarrow \hlf{l_1}!\hms{m_3}$\\
    $\{\hlf{l_2}\} \leftarrow \hlf{l_2}!\hms{m_3}$
    };
    \end{tikzpicture}
};
\draw[->] (s1) -- node[midway,fill=white,draw] {\footnotesize$\hlf{l_1}!\hms{m_2}$} (s2);
%
\node[draw, left=.75cm of s2.north west,anchor=north east] (s3) {
    \begin{tikzpicture}
    \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/isd4.png}};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_1}\} \leftarrow \varepsilon$\\
    $\{\hlf{l_2}\} \leftarrow \hlf{l_2}!\hms{m_3}$
    };
    \end{tikzpicture}
};
\draw[->] (s2) -- node[midway,fill=white,draw,rotate=270] {\footnotesize$\hlf{l_1}!\hms{m_3}$} (s3);
%
\node[draw, left=.75cm of s3.north west,anchor=north east] (s4) {
    \begin{tikzpicture}
    \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/isd4.png}};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_2}\} \leftarrow \hlf{l_2}!\hms{m_3}$
    };
    \end{tikzpicture}
};
\draw[->] (s3) -- node[midway,fill=white,draw,rotate=270] {\footnotesize$\lifelineElim_{\{\hlf{l_1}\}}$} (s4);
%
\node[draw, below=.25cm of s4,chamfered rectangle,fill=red,minimum width=1.5cm,minimum height=.5cm] (v) {\textcolor{white}{\textbf{Nok}}};
\draw[->,red] (s4) -- (v);
\end{tikzpicture}

==> images/locana_basic_fail/wtloc.tex <==
\begin{tikzpicture}
\node[draw] at (0,0) (s0) {
    \begin{tikzpicture}
    \node (int) {\includegraphics[scale=.35]{images/locana_basic_fail/isd1.png}};
    \node[right=-.25cm of int,align=left] (mu) {
    $\{\hlf{l_1}\} \leftarrow \hlf{l_1}!\hms{m_1}.\hlf{l_1}!\hms{m_2}.\hlf{l_1}!\hms{m_3}$\\
    $\{\hlf{l_2}\} \leftarrow \hlf{l_2}!\hms{m_3}$
    };
    \end{tikzpicture}
};
%
\node[draw, red] at (0,-3.9) (s1) {
\scalebox{.8}{
\begin{tikzpicture}
    \node[draw,blue] (loc_l1) {\input{images/locana_basic_fail/locana_l1}};
    \node[draw,red,below=.25cm of loc_l1] (loc_l2) {\input{images/locana_basic_fail/locana_l2}};
\end{tikzpicture}
}
};
%
\draw[->,red] (s0) -- (s1);
%
\node[draw, below=.25cm of s1,chamfered rectangle,fill=red,minimum width=1.5cm,minimum height=.5cm] (v) {\textcolor{white}{\textbf{Nok}}};
\draw[->,red] (s1) -- (v);
\end{tikzpicture}

==> images/locana_fail/wtloc/loc1.tex <==
\begin{tikzpicture}
    \node[draw,black] (s1_l2_0) {
        \begin{tikzpicture}
        \node (int) {\includegraphics[scale=.35]{images/locana_fail/wtloc/loc1_ids1.png}};
        \node[right=-.25cm of int,align=left] (mu) {
        $\{\hlf{l_1}\} \leftarrow \hlf{l_1}!\hms{m_2}$
        };
        \end{tikzpicture}
    };
    \node[draw,black, right=.75cm of s1_l2_0,chamfered rectangle,fill=red,minimum width=1.5cm,minimum height=.5cm] (v_1_l2) {\textcolor{white}{\textbf{Nok}}};
    \draw[->,red] (s1_l2_0) -- (v_1_l2);
\end{tikzpicture}

==> images/locana_fail/wtloc/loc2.tex <==
\begin{tikzpicture}
    \node[draw,black] (s1_l2_0) {
        \begin{tikzpicture}
        \node (int) {$\varnothing~~~$};
        \node[right=-.25cm of int,align=left] (mu) {
        $\{\hlf{l_2}\} \leftarrow \hlf{l_2}?\hms{m_1}.\hlf{l_2}?\hms{m_3}$
        };
        \end{tikzpicture}
    };
    \node[draw,black, below=.25cm of s1_l2_0,chamfered rectangle,fill=red,minimum width=1.5cm,minimum height=.5cm] (v_1_l2) {\textcolor{white}{\textbf{Nok}}};
    \draw[->,red] (s1_l2_0) -- (v_1_l2);
\end{tikzpicture}
